Fully Abstract and Robust Compilation and How to Reconcile the Two, Abstractly

The most prominent formal criterion for secure compilation is full abstraction, the preservation and reflection of contextual equivalence. Recent work introduced robust compilation, defined as the preservation of robust satisfaction of hyperproperties, i.e., their satisfaction against arbitrary attackers. In this paper, we initially set out to compare these two approaches to secure compilation. To that end, we provide an exact description of the hyperproperties that are robustly satisfied by programs compiled with a fully abstract compiler, and show that they can be meaningless or trivial. We then propose a novel criterion for secure compilation formulated in the framework of Mathematical Operational Semantics (MOS), guaranteeing both full abstraction and the preservation of robust satisfaction of hyperproperties in a more sensible manner.

==> Makefile <==
.PHONY: supplement clean pulp techreport

PDFLATEX = pdflatex $(OTHERFLAGS)

NAME = main

aplas:
	$(PDFLATEX) -interaction nonstopmode $(NAME)_aplas.tex
	-bibtex $(NAME)_aplas
	$(PDFLATEX) -interaction nonstopmode $(NAME)_aplas.tex
	$(PDFLATEX) -interaction nonstopmode $(NAME)_aplas.tex

arxiv:
	$(PDFLATEX) -interaction nonstopmode $(NAME)_arxiv.tex
	-bibtex $(NAME)_arxiv
	$(PDFLATEX) -interaction nonstopmode $(NAME)_arxiv.tex
	$(PDFLATEX) -interaction nonstopmode $(NAME)_arxiv.tex

mfps:
	$(PDFLATEX) -interaction nonstopmode $(NAME)_mfps.tex
	-bibtex $(NAME)_mfps
	$(PDFLATEX) -interaction nonstopmode $(NAME)_mfps.tex
	$(PDFLATEX) -interaction nonstopmode $(NAME)_mfps.tex

clean:
	rm -f *.log *.aux *.upb *.upa *.bbl *.html *.css *.dvi *.blg *.out *.synctex

# You can get pulp here: https://github.com/dmwit/pulp
PULP = "$(shell which pulp || echo \"$(HOME)\"~/.cabal/bin/pulp)"

pulp:
	rm -f $(NAME).log
	-$(PDFLATEX) -interaction nonstopmode $(NAME) &> /dev/null
	-bibtex $(NAME)
	-$(PDFLATEX) -interaction nonstopmode $(NAME) &> /dev/null
	-$(PDFLATEX) -interaction nonstopmode $(NAME) &> /dev/null
	-$(PULP) $(NAME).log | grep -v "/usr/share/texmf-dist/tex/"

DATE = "$(shell date +'%Y-%m-%d--%H-%M')"


